Rovibrational-Specific QCT and Master Equation Study on $\text{N}_2(\text{X}^1\Sigma_g^+)$+$\text{O}({}^3\text{P})$ and $\text{NO}(\text{X}^2\Pi)$+$\text{N}({}^4\text{S})$ Systems in High-Energy Collisions

This work presents a detailed investigation of the energy transfer and dissociation mechanisms in $\text{N}_2(\text{X}^1\Sigma_g^+)$+$\text{O}({}^3\text{P})$ and $\text{NO}(\text{X}^2\Pi)$+$\text{N}({}^4\text{S})$ systems using rovibrational-specific quasi-classical trajectory (QCT) and master equation analyses. The complete set of state-to-state kinetic data, obtained via QCT, allows for an in-depth investigation of the Zel'dovich mechanism leading to the formation of $\text{NO}$ molecules at microscopic and macroscopic scales. The master equation analysis demonstrates that the low-lying vibrational states of $\text{N}_2$ and $\text{NO}$ have dominant contributions to the $\text{NO}$ formation and the corresponding extinction of $\text{N}_2$ through the exchange process. For the considered temperature range, it is found that while nearly 50% of the dissociation processes for $\text{N}_2$ and $\text{NO}$ occurs in the molecular quasi-steady-state (QSS) regime, the amount of the Zel'dovich reaction is zero. Using the QSS approximation to model the Zel'dovich mechanism leads to an overestimation of $\text{NO}$ production by more than a factor of 4 in the high-temperature range. The breakdown of this well-known approximation has profound consequences for the approaches that heavily rely on the validity of QSS assumption in hypersonic applications. The investigation of the rovibrational state population dynamics reveals substantial similarity among different chemical systems for the energy transfer and the dissociation processes, providing promising physical foundations for the use of reduced-order strategies to other chemical systems without significant loss of accuracy.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
